Haptic Interactions for Extended Reality

This research investigates whether the interaction methods of XR headsets can be improved by using haptic feedback. As a first and most common technique, indirect interactions are considered. Indirect interactions correspond to manipulations of virtual objects from a virtual distance using pre-defined hand gestures. As a second interaction technique, direct interaction (namely DIM) has been implemented where the user manipulates objects by virtually touching these with their hands. A third interaction method extends the previous one with haptic feedback (namely HEDIM). These 3 methods are compared with each other based on objective and subjective user tests, also taking into account financial considerations. This research concludes that the DIM improves upon the standard indirect method. Additionally, it has been observed that haptic feedback could enhance the DIM in specific situations. Nevertheless, when considering the current financial cost, our subjects were not convinced of the small improvements haptic feedback brings.

==> Bibliografie.tex <==
\renewcommand\bibname{References}
\bibliography{referenties}


==> ICCE 2023 - arxiv/Bibliografie.tex <==
\renewcommand\bibname{References}
\bibliography{referenties}


==> ICCE 2023 - arxiv/acronyms.tex <==
%\acrlong{gcd}  
%\acrshort{gcd}  
%\acrfull{lcm}  
%\newacronym{gcd}{GCD}{Greatest Common Divisor- test acronym}

\newacronym{ar}{AR}{Augmented Reality}
\newacronym{hmd}{HMD}{Head-Mounted Display}
\newacronym{vr}{VR}{Virtual Reality}
\newacronym{mr}{MR}{Mixed Reality}
\newacronym{xr}{XR}{eXtended Reality}
\newacronym{av}{AV}{Augmented Virtuality}
\newacronym{sr}{SR}{Simulated Reality}
\newacronym{vhmr}{VHMR}{Visio-Haptic Mixed Reality}
\newacronym{nasa}{NASA}{National Aeronautics and Space Administration}
\newacronym{marta}{MARTA}{Mobile Augmented Reality Technical Assistance}
\newacronym{dof}{DoF}{Degrees of Freedom}
\newacronym{fps}{FPS}{Frames Per Second}
\newacronym{rfid}{RFID}{Radio-Frequency IDentification}
\newacronym{qos}{QoS}{Quality-of-Service}
\newacronym{qoe}{QoE}{Quality-of-Experience}
\newacronym{jet}{JET}{Joint European Torus}
\newacronym{afrl}{AFRL}{United States Air Force Research Laboratory}
\newacronym{imu}{IMU}{Inertial Measurement Unit}
\newacronym{dll}{dll}{Dynamic-Link Library}
\newacronym{fov}{FoV}{Field of View}
\newacronym{hpu}{HPU}{Holographic Processing Unit}
\newacronym{srg}{SRG}{Surface Relief Grating}
\newacronym{vhg}{VHG}{Volumetric Holographic Grating}
\newacronym{lra}{LRA}{Linear Resonant Actuators}
\newacronym{ipd}{IPD}{Inter-Pupillary Distance}
\newacronym{gdpr}{GDPR}{General Data Protection Regulation}
\newacronym{ssq}{SSQ}{Simulator Sickness Questionnaire}
\newacronym{sdgs}{SDGs}{Sustainable Development Goals}
\newacronym{dim}{DIM}{Direct Interaction Method}
\newacronym{hedim}{HEDIM}{Haptic Enhanced Direct Interaction Method}
\newacronym{idlab}{IDLAB}{Internet Technology And Data Science Lab}
\newacronym{mreq}{MREQ}{Mixed Reality Experience Questionnaire}

